Spectral Approach to Verifying Non-linear Arithmetic Circuits

This paper presents a fast and effective computer algebraic method for analyzing and verifying non-linear integer arithmetic circuits using a novel algebraic spectral model. It introduces a concept of algebraic spectrum, a numerical form of polynomial expression; it uses the distribution of coefficients of the monomials to determine the type of arithmetic function under verification. In contrast to previous works, the proof of functional correctness is achieved by computing an algebraic spectrum combined with a local rewriting of word-level polynomials. The speedup is achieved by propagating coefficients through the circuit using And-Inverter Graph (AIG) datastructure. The effectiveness of the method is demonstrated with experiments including standard and Booth multipliers, and other synthesized non-linear arithmetic circuits up to 1024 bits containing over 12 million gates.

==> abstract.tex <==
\begin{table*}[t]
\scriptsize
\centering
\caption{Evaluation of word-level abstraction using algebraic spectrum. Multiplications in $F_{1}$ and $F_{2}$ are implemented using CSA-multiplier. $F_{3}$ uses radix-4 Booth-multiplier.}
\label{tbl:abstract}
\begin{tabular}{|l|c|c|r|c|c|r|c|c|c|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Benchmarks\\ 128-bit\end{tabular}} & \multicolumn{3}{c|}{This Approach} & \multicolumn{3}{c|}{\cite{yu:2016-abstraction}} & \multicolumn{3}{c|}{\cite{soeken:2015simulationgraph}} \\ \hline
Function (128-bit) & \multicolumn{1}{l|}{\textit{Mult}} & \multicolumn{1}{l|}{\textit{Add}} & \multicolumn{1}{l|}{Runtime} & \multicolumn{1}{l|}{\textit{Mult}} & \multicolumn{1}{l|}{\textit{Add}} & \multicolumn{1}{l|}{Runtime} & \multicolumn{1}{l|}{\textit{Mult}} & \multicolumn{1}{l|}{\textit{Add}} & \multicolumn{1}{l|}{Runtime} \\ \hline
\textit{$F_{1}$=A$\times$B+C (CSA)} & 1 & 1 & 0.45 s & 1 & 1 & 23760 s & 0 & 0 & - \\ \hline
\textit{$F_{2}$=A$\times$B+A$\times$C (CSA)} & 2 & 1 & 1.03 s & 2 & 1 & 48560 s & 0 & 0 & - \\ \hline
\textit{$F_{3}$=A$\times$B+C (Booth)} & - & - & \multicolumn{1}{c|}{-} & - & - & \multicolumn{1}{c|}{-} & 0 & 0 & - \\ \hline
\end{tabular}
\end{table*}

==> abstraction_example.tex <==
\vspace{-2mm}
\subsection{Illustrative Example}\label{sec:example}
 We illustrate the concept of our abstraction using a simple ALU design (Figure \ref{fig:alu}). The inputs $A,B,C$ are 4-bit wide and $P$ is 8-bit wide, and $f_{C}$ is a majority function. 
 %Note that $f_{C}$ can be any combinational function. The control logic will be extracted by "decomposition"
 $M1, M2$ are 4-bit multipliers and $ADD$ is an 8-bit adder. The output of two multipliers are selected by the $f_{C}$. Note that all components in the ALU are gate-level. The output signature is $ \scriptstyle F =\scriptstyle \sum\limits_{i=0}^8 f_{i}2^i$. 

 The first identified $word~cut$ is $\mathcal{C}_{1}$. Using Algorithm 1, $\mathcal{C}_{1}$ is identified as a \textit{multi-word} linear expression. The word of  $word~cut$ $\mathcal{C}_{1}$ is associated with $M1, M2$, $f_{C}$, and primary input $P$. The signals associated with $P$ are all primary inputs and the signals associated with $\mathcal{W}_{1}$ include $M1, M2$ and $f_{C}$. Hence, the word $P$ and $\mathcal{W}_{1}$ can be easily abstracted in $cut~\mathcal{C}_{1}$. 
The next $word~cut$ is identified as $\mathcal{C}_{2}$. This $word~cut$ is different than $\mathcal{C}_{1}$ since there is a MUX operation. The function of cut $\mathcal{C}_{2}$ is $(1-f_{C})\mathcal{W}_{2}+f_{C}\mathcal{W}_{3}$. Note that the expression is $flattened$ to maximize the cancellations. Hence, the expression of $c_{2}$ in our process is $\mathcal{W}_{2}-\mathcal{W}_{2}f_{C}+\mathcal{W}_{3}f_{C}$. The $step~5$ in Algorithm 1 recognizes the decomposable part $-\mathcal{W}_{2}f_{C}+\mathcal{W}_{3}f_{C}$, and returns $-\mathcal{W}_{2}+\mathcal{W}_{3}$. Then, the returned expression is identified in $step~11$ as a non-linear \textit{multi-word}. The word $\mathcal{W}_{2}$ and $\mathcal{W}_{3}$ come from two different multipliers. Therefore, the associated graph is able to classify these two words from the expression. As we mentioned in $step~5$, the non-decomposable expression, in case $\mathcal{W}_{2}$, is a word expression. This is the reason why our algorithm checks both decomposable and non-decomposable sub-expressions.
The process stops when the rewriting reaches the PIs.

\begin{figure}[t] 
\begin{center}
\includegraphics[scale=0.28]{../figs/example.eps}
\caption{ALU design with multiplier $M_{1},M_{2}$, adder $ADD$, and $f_{C}=MAJ(n1,n2,n3)$ }
\vspace{-2mm}
\label{fig:alu}
\end{center}
\end{figure}

==> booth.tex <==
\begin{table}[!htb]
\scriptsize
\centering
\caption{Runtime of extracting the specification of the radix-4 Booth multiplier. \textit{*MO} = Memory out of 8GB.}
\label{tbl:booth}
\begin{tabular}{|c|c|c|r|r|}
\hline
\multirow{2}{*}{\# bits} & \multicolumn{2}{c|}{\cite{ciesielski2015verification}} & \multicolumn{2}{c|}{This approach} \\ \cline{2-5} 
 & Pre-syn (s) & Post-syn (s) & \multicolumn{1}{c|}{Pre-syn (s)} & \multicolumn{1}{c|}{Post-syn (s)} \\ \hline
64 & MO & MO & 0.05 & 0.06 \\ \hline
128 & - & - & 0.51 & 6.97 \\ \hline
256 & - & - & 1.95 & 22.70 \\ \hline
512 & - & - & 5.50 & \multicolumn{1}{c|}{-} \\ \hline
\end{tabular}
\end{table}


==> extras.tex <==

%The spectrum for each polynomial is represented as a collection of individual spectra $S_k$ for all possible values of $k$ that the monomials may take during rewriting, even if the final polynomial is composed of monomials with a fixed number of variables. 

%In short, the spectrum gives information about the {\it form} of the polynomial (type of the arithmetic function) and not about the actual variables or the composition of the operands in terms of those variables. This "disambiguation" will need to be resolved separately. An important insight into the type of the function can be gained by analyzing the number of variables in the polynomial representing the function.  
%For example, the polynomial with $M$ monomials, each containing two different variables (for a total of $2M$ variables) cannot possibly be a two-operand multiplier, even if such a polynomial maps into the same spectrum, because the multiplier with $M$ monomials can only contain $sqrt(M)$ variables. This kind of analysis must complement the analysis of the spectrum when trying to determine the function implemented by the circuit; this is beyond the scope of this paper.
%
%However, we use algebraic spectrum for the purpose of analyzing {\it arithmetic functions} and not arbitrary polynomials. It can be effective in this context as an abstract representation. Specifically, we can define an equivalence relation between two polynomials that have the same spectrum and create a {\it class} of equivalent arithmetic circuits under this equivalence relation (augmented with analysis of the variables). In this context, the goal of arithmetic verification, as presented in this work, is to determine if the given circuit belongs to a given class, for example a two-operand multiplier, three-operand adder, a MAC, etc. 

%The method currently concentrates on monolithic arithmetic circuits, i.e., those, whose specification polynomial, $Sig_{in}$, contains monomials with the same number of variables. For example, in an adder all monomials are single-variable, and in an $k-$input multipliers all monomials are $k-$variable product terms. This is in contrast to other circuits, such as a fused multiply/add circuit, which contain both single-variable and two-(or more-)variable monomials. 
%In the fused multiply/add circuit discussed in Section \ref{sec:spectral-method}, Figure \ref{fig:mac-spectrum} two spectra were used to represent the circuit, each for the corresponding number of monomial variables. However, other representations are also possible, for example by deriving a single spectrum, without distinguishing between the number of variables and superimposing the two spectra. This and other problems give an interesting direction for our future work.
%Currently this work applies mostly to verification of {\it correct} circuits, in which the coefficients of the polynomials are $C_i=2^k$. 

==> figs/abstraction_example.tex <==
\vspace{-2mm}
\subsection{Illustrative Example}\label{sec:example}
 We illustrate the concept of our abstraction using a simple ALU design (Figure \ref{fig:alu}). The inputs $A,B,C$ are 4-bit wide and $P$ is 8-bit wide, and $f_{C}$ is a majority function. 
 %Note that $f_{C}$ can be any combinational function. The control logic will be extracted by "decomposition"
 $M1, M2$ are 4-bit multipliers and $ADD$ is an 8-bit adder. The output of two multipliers are selected by the $f_{C}$. Note that all components in the ALU are gate-level. The output signature is $ \scriptstyle F =\scriptstyle \sum\limits_{i=0}^8 f_{i}2^i$. 

 The first identified $word~cut$ is $\mathcal{C}_{1}$. Using Algorithm 1, $\mathcal{C}_{1}$ is identified as a \textit{multi-word} linear expression. The word of  $word~cut$ $\mathcal{C}_{1}$ is associated with $M1, M2$, $f_{C}$, and primary input $P$. The signals associated with $P$ are all primary inputs and the signals associated with $\mathcal{W}_{1}$ include $M1, M2$ and $f_{C}$. Hence, the word $P$ and $\mathcal{W}_{1}$ can be easily abstracted in $cut~\mathcal{C}_{1}$. 
The next $word~cut$ is identified as $\mathcal{C}_{2}$. This $word~cut$ is different than $\mathcal{C}_{1}$ since there is a MUX operation. The function of cut $\mathcal{C}_{2}$ is $(1-f_{C})\mathcal{W}_{2}+f_{C}\mathcal{W}_{3}$. Note that the expression is $flattened$ to maximize the cancellations. Hence, the expression of $c_{2}$ in our process is $\mathcal{W}_{2}-\mathcal{W}_{2}f_{C}+\mathcal{W}_{3}f_{C}$. The $step~5$ in Algorithm 1 recognizes the decomposable part $-\mathcal{W}_{2}f_{C}+\mathcal{W}_{3}f_{C}$, and returns $-\mathcal{W}_{2}+\mathcal{W}_{3}$. Then, the returned expression is identified in $step~11$ as a non-linear \textit{multi-word}. The word $\mathcal{W}_{2}$ and $\mathcal{W}_{3}$ come from two different multipliers. Therefore, the associated graph is able to classify these two words from the expression. As we mentioned in $step~5$, the non-decomposable expression, in case $\mathcal{W}_{2}$, is a word expression. This is the reason why our algorithm checks both decomposable and non-decomposable sub-expressions.
The process stops when the rewriting reaches the PIs.

\begin{figure}[t] 
\begin{center}
\includegraphics[scale=0.28]{../figs/example.eps}
\caption{ALU design with multiplier $M_{1},M_{2}$, adder $ADD$, and $f_{C}=MAJ(n1,n2,n3)$ }
\vspace{-2mm}
\label{fig:alu}
\end{center}
\end{figure}
